CodeAgent: Autonomous Communicative Agents for Code Review

Code review, which aims at ensuring the overall quality and reliability of software, is a cornerstone of software development. Unfortunately, while crucial, Code review is a labor-intensive process that the research community is looking to automate. Existing automated methods rely on single input-output generative models and thus generally struggle to emulate the collaborative nature of code review. This work introduces \tool{}, a novel multi-agent Large Language Model (LLM) system for code review automation. CodeAgent incorporates a supervisory agent, QA-Checker, to ensure that all the agents' contributions address the initial review question. We evaluated CodeAgent on critical code review tasks: (1) detect inconsistencies between code changes and commit messages, (2) identify vulnerability introductions, (3) validate code style adherence, and (4) suggest code revision. The results demonstrate CodeAgent's effectiveness, contributing to a new state-of-the-art in code review automation. Our data and code are publicly available (\url{https://github.com/Code4Agent/codeagent}).

==> sections/7.Discussion.tex <==
\section{Limitation and Discussion}

==> sections/preliminary.tex <==
\section{Preliminary Study: Dynamic Programming}\label{sec:reasoning}
% \subsection{ in Code Review} 

%Advanced Dynamic Programming Formulation for \tool{} Code Review

% Inspired by \cite{feng2023towards}, we provide a preliminary study in Appendix Sec xxx.

In this section, we adapt the general settings of dynamic programming (DP) to the context of code review, particularly focusing on the tasks of consistency analysis, vulnerability analysis, and format analysis. We posit that large language models (LLMs) with Chain of Thought (CoT) can effectively emulate dynamic programming for these complex code review tasks.

\subsubsection{Definitions of Dynamic Programming}
Dynamic programming (DP) is a method widely used in decision-making problems, and its applicability extends to the domain of code review. The fundamental principle of DP in this context is to decompose the complex problem of code review into smaller, manageable subproblems. These subproblems represent different aspects of the code review process, such as consistency analysis, vulnerability analysis, and format analysis, ensuring significant overlap and interconnection for efficient problem-solving.

Formally, we adapt the DP algorithm for code review with these key components:
\begin{itemize}
    \item \textbf{State Space} $\gI$: Represents the set of subproblems in code review. Each state signifies a specific aspect like checking consistency between code and documentation, identifying potential security vulnerabilities, or analyzing code formatting.
    
    \item \textbf{Transition Function} $T$: Defines the relationship between the subproblems. It determines how a subproblem's solution can be derived from the solutions of preceding subproblems, relevant to the specific aspect of code review it represents.
    
    \item \textbf{Aggregation Function} $A$: Combines the results of all subproblems to form a comprehensive code review report.
\end{itemize}



Given a code review task characterized by a sequence of inputs (code segments, documentation, etc.), the DP algorithm in \tool{} operates as follows:
\begin{enumerate}
    \item Each subproblem in the state space is addressed sequentially, following the partial order dictated by code review logic.
    \item The transition function applies LLMs with CoT reasoning to solve each subproblem, utilizing the context provided by previously solved subproblems.    
    \item The aggregation function then synthesizes the individual solutions into a final, coherent code review output, covering all aspects of consistency, vulnerability, and formatting.
\end{enumerate}

Specifically, we input $N$ sequences, which are donated as $\vs^{(1)},\cdots,\vs^{(N)}$ to represent the size

By integrating dynamic programming with LLMs and CoT reasoning, \tool{} provides an efficient and effective framework for automating complex code review tasks. This approach not only streamlines the review process but also ensures comprehensive and accurate assessments of code quality and security.


